V-Formation via Model Predictive Control

We present recent results that demonstrate the power of viewing the problem of V-formation in a flock of birds as one of Model Predictive Control (MPC). The V-formation-MPC marriage can be understood in terms of the problem of synthesizing an optimal plan for a continuous-space and continuous-time Markov decision process (MDP), where the goal is to reach a target state that minimizes a given cost function. First, we consider ARES, an approximation algorithm for generating optimal plans (action sequences) that take an initial state of an MDP to a state whose cost is below a specified (convergence) threshold. ARES uses Particle Swarm Optimization, with adaptive sizing for both the receding horizon and the particle swarm. Inspired by Importance Splitting, the length of the horizon and the number of particles are chosen such that at least one particle reaches a next-level state. ARES can alternatively be viewed as a model-predictive control (MPC) algorithm that utilizes an adaptive receding horizon, aka Adaptive MPC (AMPC). We next present Distributed AMPC (DAMPC), a distributed version of AMPC that works with local neighborhoods. We introduce adaptive neighborhood resizing, whereby the neighborhood size is determined by the cost-based Lyapunov function evaluated over a global system state. Our experiments show that DAMPC can perform almost as well as centralized AMPC, while using only local information and a form of distributed consensus in each time step. Finally, inspired by security attacks on cyber-physical systems, we introduce controller-attacker games (CAG), where two players, a controller and an attacker, have antagonistic objectives. We formulate a special case of CAG called V-formation games, where the attacker's goal is to prevent the controller from attaining V-formation. We demonstrate how adaptation in the design of the controller helps in overcoming certain attacks.

==> cutoff.tex <==
\subsection{Stochastic reachability problem}
The problem of whether we can go from a random flock to a V-formation can be posed as a reachability question, where the reachability goal is the set of states representing a V-formation. A key assumption in~\cite{LukinaEHBYTSG17} was that the reachability goal can be specified as $J(s) \leqslant \varphi$, where $J$ is a fitness function   
that assigns a non-negative real (fitness) value to each state $s$, and $\varphi$ is a small positive constant. 
%Moreover, $J$ was defined so that $J(s)\,{<}\,{\varphi}$, for a small $\varphi$, for exactly those states $s$ that correspond to a V-formation. {This is mentioned after eq.2} 
%Each state of $\mathcal{M}$ is represented by a fitness function reflecting essential motives for birds to fly in a V-formation in the first place.

The fitness of a state was determined by the following three terms: 
%% using three terms that measured if: (a)~birds have a clear visual field not blocked by any bird in front of them (\emph{clear view}); (b)~birds have the same velocity (\emph{velocity matching}); and
%% (c)~birds are located in space so that they are positioned in the upwash region of the bird(s) in front of them (\emph{upwash benefit}). 
\begin{itemize}
	\vspace*{-1.4mm}\item \emph{Clear View}. A bird's visual field is a cone with 
    angle $\theta$ that can be blocked by the wings of other birds. 
    The clear-view metric is defined by accumulating the percentage of a bird's visual 
    field that is blocked by other birds. $CV(s)$ for flock state $s$ is the sum of the clear-view
    metric of all birds. The minimum value of $\CV$ 
    is $\CV^*{=}\,0$, and this value is attained in a perfect V-formation where all birds have clear view.
    
	\vspace*{1mm}\item \emph{Velocity Matching}. $\VM(s)$ for flock state $s$ is defined as the  
	difference between the velocity of a given bird and all other birds, 
    summed up over all birds in the flock. The minimum
    value for $\VM$ is $\VM^*{=}\,0$, and this value is attained in a perfect
    V-formation where all birds have the same 
    velocity.
    
	\vspace*{1mm}\item \emph{Upwash Benefit}. The trailing upwash is 
    generated near the wingtips of a bird, while downwash is generated near 
    the center of a bird.  An upwash measure $um$ is defined on the 2D space using a 
    Gaussian-like model that peaks at the appropriate upwash and downwash regions. 
    %{Jesse: I commented this out as $um$ could be larger than 1 due to downwash} By design, the maximum $um$ for a bird is~1. 
    For bird~$i$ with upwash $um_i$, the upwash-benefit metric $\UB_i$ is defined as
    $1\,{-}um_i$, and $\UB(s)$ for flock state $s$ is the sum of all $\UB_i$ for $1\leqslant i \leqslant B$.
    The upwash benefit $\UB(s)$ in V-formation is $\UB^*\,{=}\,1$, as all birds, except for the leader, have 
    minimum upwash-benefit metric ($\UB_i=0, um_i=1$),
    while the leader has upwash-benefit metric of $1$ ($\UB_i=1, um_i=0$).
\end{itemize}

\subsection{Cost function}
\noindent{}Given the above metrics, the overall fitness (cost) metric $J$ 
is of a sum-of-squares combination of $\VM$, $\CV$, and $\UB$ defined as follows:
\vspace*{-1mm}
\begin{align}
J(s) = (\CV(s)-\CV^*)^2 + (\VM(s)-\VM^*)^2 +(\UB(s)-\UB^*)^2.
\label{eq:fitness}
\end{align}
A state $s^{*}$ is considered to be a V-formation whenever $J(s^{*})\,{\leqslant}\,\varphi$, for a small positive threshold $\varphi$.


==> vgame.tex <==
\begin{figure}[t]
 \centering
  \includegraphics[width=.495\textwidth]{figures/numbering}
  \includegraphics[width=.495\textwidth]{figures/remove2and5}
  \caption{Left: numbering of the birds. Right: configuration after removing Bird 2 and 5. The red-filled circle and two protruding line segments represent a bird's body and wings. Arrows represent bird velocities. Dotted lines illustrate clear-view cones. A brighter/darker background color indicates a higher upwash/downwash.}
  \label{fig:numbering}
  \vspace{-3ex}
 \end{figure}

\begin{table}[ht]
\centering
\caption {Results of 2,000 game executions for removing 1 bird with $h_{\mathit{max}}\,{=}\,5$,  $m\,{=}\,40$}
\vspace*{-1ex}
    \begin{tabular}{lcccccccccc}
    \toprule
		&&& Ctrl. success rate, \% &&& Avg. convergence duration &&& Avg. horizon\\ \midrule
    Bird 4  && & $99.9$           && & $12.75$  &&& $3.64$                            \\
    Bird 3  && & $99.8$           && & $18.98$  &&& $4.25$                            \\
    Bird 2  && & $100$           && & $10.82$  &&& $3.45$                            \\ \bottomrule
    \end{tabular}
\label{tab:resRemoveOne}
%\vspace*{-3ex}
\end{table}

%\vspace*{-4ex}
\begin{table}[ht]
%\vspace*{-3mm}
% 	\scriptsize
	\centering
	\caption{Results of 2,000 game executions for removing 2 birds with $h_{\mathit{max}} \,{=}\,5$, $m\,{=}\,30$}
	\begin{tabular}{lccccccccccc}
		\toprule
		&&& Ctrl. success rate, \% &&& Avg. convergence duration &&& Avg. horizon\\
      	\midrule
        Birds 2 and 3 & & &$0.8$ & & &$25.18$&&&$4.30$\\
        Birds 2 and 4 & & &$83.1$ & & &$11.11$ &&&$2.94$\\
        Birds 2 and 5 & & &$80.3$ & & &$9.59$ &&&$2.83$\\
        Birds 2 and 6 & & &$98.6$ & & &$7.02$ &&&$2.27$\\
        Birds 3 and 4 & & &$2.0$ & & &$22.86$ &&&$4.30$\\
        Birds 3 and 5 & & &$92.8$ & & &$11.8$ &&&$3.43$\\
		\bottomrule
\end{tabular}
\label{tab:resRemoveTwo}
%\vspace*{-3ex}
\end{table}

\begin{table}[t]
%\vspace*{-3mm}
% 	\scriptsize
	\centering
	\caption{Results of 2,000 game executions for random displacement and AMPC attacks with $h_{\mathit{max}}\,{=}\,5$ and $m\,{=}\,40$ (attacker runs for 20 steps)}
	\begin{tabular}{cccccccccccc}  
		\toprule
		Range of noise &&& Ctrl. success rate, \% &&& Avg. convergence duration &&& Avg. horizon\\
      	\midrule
        &&&\multicolumn{7}{c}{Random displacement game}\\
        \cmidrule(l){3-10}
        $[0,0.50]\times[0,2\pi]$ & & &$99.9$ & & &$3.33$ &&&$1.07$\\
        $[0,0.75]\times[0,2\pi]$ & & &$97.9$ & & &$3.61$ &&&$1.11$\\
        $[0,1.00]\times[0,2\pi]$ & & &$92.3$ & & &$4.14$ &&&$1.18$\\
 		\cmidrule(l){3-10}
        &&&\multicolumn{7}{c}{AMPC game}\\
        \cmidrule(l){3-10}
        $[0,0.50]\times[0,2\pi]$  && & $97.5$    &&& $4.29$ &&& $1.09$\\
        $[0,0.75]\times[0,2\pi]$  && & $63.4$    &&& $5.17$ &&& $1.23$\\
        $[0,1.00]\times[0,2\pi]$  && & $20.0$    &&& $7.30$ &&& $1.47$\\
		\bottomrule
\end{tabular}
\label{tab:resRandomNoise}
%\vspace*{-3ex}
\end{table}


